Data-driven Super-resolution on a Tactile Dome

While tactile sensor technology has made great strides over the past decades, applications in robotic manipulation are limited by aspects such as blind spots, difficult integration into hands, and low spatial resolution. We present a method for localizing contact with high accuracy over curved, three dimensional surfaces, with a low wire count and reduced integration complexity. To achieve this, we build a volume of soft material embedded with individual off-the-shelf pressure sensors. Using data driven techniques, we map the raw signals from these pressure sensors to known surface locations and indentation depths. Additionally, we show that a finite element model can be used to improve the placement of the pressure sensors inside the volume and to explore the design space in simulation. We validate our approach on physically implemented tactile domes which achieve high contact localization accuracy ($1.1mm$ in the best case) over a large, curved sensing area ($1,300mm^2$ hemisphere). We believe this approach can be used to deploy tactile sensing capabilities over three dimensional surfaces such as a robotic finger or palm.

==> method.tex <==
\section{Data Collection Methodology}

We want to find a mapping between the five pressure sensor readings and the location of an indentation. To collect data on the fabricated tactile domes, we designed an indenter machine with five degrees of freedom (DOF) to probe at specified locations and depths along the dome's surface with varying angles from the surface normal (Fig.~\ref{fig:indenter_machine}). The indenter machine is composed of a planar stage (Marzhauser LStep) where we mount our tactile dome on top of a rotating base. We mount a position controlled linear actuator (Physik Instrumente M-235-5DD) on a revolute joint directly above the dome. The linear actuator is equipped with a $6mm$ diameter aluminum hemispherical tip. The only unaccounted DOF is a revolute joint around the tool tip axis. In this study all indentations are performed with the linear actuator positioned normal to the dome surface. 

In order to collect training data, the tactile dome is sampled at equidistant locations along its surface. To achieve this uniform distribution over a spherical surface, a mapping scheme \cite{rocsca2010new} is used to project a two dimensional regular grid $(A,B)$ onto the dome's hemispherical surface $(x,y,z)$. Using $A,B \in [-15,15]$ results in a mapping that almost completely covers our three dimensional surface. Note that this $(A,B)$ space is dimensionless. The grid used is 16x16, hence we sample along 256 different positions on the surface of the dome for training. At each location, the probe is positioned normal to the surface and a first ``non-touch'' data point was recorded before the linear actuator tip made contact with the dome surface. Subsequently, the actuator indented the surface and recorded data at the predefined depths from $0$ to $3mm$ in $0.5mm$ intervals. 

To collect a test dataset, an identical procedure is followed but indentation locations are randomly sampled from our two dimensional $(A,B)$ space. We collect data on 100 random locations. The test dataset locations, while generated randomly within our $(A,B)$ space, are repeated for all ten sensor configuration cases (both real and simulated) for consistency.  

For each measurement $i$ we recorded the data in a tuple of the form $\Phi_i = (A,B,d_i,r_i^1,....,r_i^5)$ where $(A,B)$ is the location of the indentation before being mapped to the dome surface, $d_i$ is the depth of the measurement, and $r_i^1,....,r_i^5$ are the readings of the five pressure sensors. These tuples are used as described in the learning algorithm section. 

This method is applied to data collection for both the physical and simulated model of the tactile dome. 




==> simulation.tex <==
\section{Simulation}


The purpose of developing a simulated model of our tactile dome is to have the ability to iterate and evaluate sensor configurations to improve the localization performance without the need to build the physical sensor. 

As mentioned before, an important design parameter is the placement of the pressure sensors embedded inside the volume of material. This space can be explored purely in simulation, analyzing the pressure distribution and generating synthetic datasets to evaluate the final performance. 

We use a quasi-static, ABAQUS Standard simulation to generate both training and testing data. The indentations are performed with a $6mm$ diameter, hemispherical, rigid body at the same locations as on the physical tactile dome, normal to its surface. The indenter interacts with the tactile dome's surface with an estimated friction coefficient of 0.8. We input the Vytaflex 20 experimental stress-strain data into Abaqus and the material properties were predicted using a Marlow curve fitting model.

To simplify the model, we make the following assumptions:
\begin{itemize}
\item The tactile dome's polymer is perfectly bonded to all of the components it interfaces with during casting.
\item The compliances of the ABS base, Takktile sensor housing, and Takktile circuit are ignored. These components are treated as infinitely stiff compared to the polymer.
\item The Takktile sensor samples pressure at its air-vent hole, which is an opening to the barometer's pressure-sensing elastomer/ Wheatstone bridge. The elastomer is assumed to have the same properties as Vytaflex 20.
\end{itemize}

The first two assumptions enable us to dis-include the ABS base, Takktile sensor housing, and Takktile circuit from the simulation in order to reduce computational time and complexity. To compensate, a zero-displacement constraint in the X-Y-Z directions is applied on the surfaces where the polymer interacts with these components. It should be noted that these surfaces are not fixed in rotation to ensure that the simulation is not over-constrained. 

To reproduce the interaction between the tactile dome and the sensor, five thin, cylindrical bodies are attached to the dome's air-vent holes via a 'tie' constraint, representing perfect bonding of Vytaflex 20. The opposing cylindrical faces are fixed in the X-Y-Z directions to mimic the attachment to the Takktile boards' surfaces. The cylinders allow us to sample at a location that is not a boundary condition such that we generate a realistic output. Pressure data is sampled at the surface between the cylindrical bodies and the tactile dome.  

In order to shorten the computational time required for the solution to converge, data is collected over half of the sensor and mirrored about the line of symmetry (Fig~\ref{fig:distributions}). The dome and five bodies are modeled with a first-order mesh with hybrid elements due to the incompressible properties of Vytaflex 20 and the curved geometry. We ran a mesh convergence study using case three and determined that a 10-node, C10D4i mesh yields similar trends as a 4-node C3D4H mesh (Fig.~\ref{mesh_10}). We thus used the 4-node mesh in order to decrease the simulation run time.  


\begin{figure}[t]
\setlength{\tabcolsep}{0mm}
\begin{tabular}{cc}
\subfloat[C3D4H mesh] {\label{mesh_4}
\includegraphics[clip, trim=0.4cm 0.5cm 0.5cm 0.3cm, width=0.49\columnwidth]{images/4node.pdf}}\hfill &  \subfloat[C10D4i mesh] {\label{mesh_10}
\includegraphics[clip, trim=0.4cm 0.5cm 0.5cm 0.3cm, width=0.49\columnwidth]{images/10node.pdf}}\\
\end{tabular}
\caption{Comparison between simulations ran using a C3D4H mesh (\ref{mesh_4}) and a C10D4i mesh (\ref{mesh_10}) on Case 1. The graph represents the pressure distribution among the five Takktile sensors as we indent along the symmetry line. Both graphs show similar trends with slightly different absolute values for the reported pressure.}
\label{fig:mesh_study}
\end{figure}



